Convergence of Density Operators and Security of Discrete Modulated CVQKD Protocols

This communication deals with the problem of bounding the approximation error on weak convergence of mixed coherent state towards a Gaussian thermal state. In the context of CVQKD with discrete modulation, we develop expressions for two specific cases. The first one is the distance between the Gaussian equivalent bipartite state and a reference Gaussian modulated (GG02) and the second one is for the trace distance between the constellation and a thermal state with same photon number. Since, in the convex set of density operators, weak convergence implies convergence in the trace norm, knowing how fast the sequence gets close to the equivalent Gaussian state has implication on the security of QKD Protocols. Here we derive two bounds on the $L_1$ distance, one of them related with an energy test that can be used in the security proof.

==> files/sec01.tex <==
\section{Introduction}

% Tha task of communicating with information theoretic security is possible by applying \textit{on-time-pad} cyphers, which require the distant parties (Alice and Bob) to possess a new random binary secret key for each message to be sent. Quantum key Distribution (QKD) protocols provides a method for such keys to be generated with security guaranteed by the laws of quantum mechanics, which ensures that the action of an eavesdropper (Eve) can not be inconspicuous.

Since its proposal, quantum key distribution protocols have 
